Low temperature acoustic polaron localization

We calculate the properties of an acoustic polaron in three dimensions in thermal equilibrium at a given low temperature using the path integral Monte Carlo method. The specialized numerical method used is described in full details, thus complementing our previous paper [R. Fantoni, Phys. Rev. B {\bf 86}, 144304 (2012)], and it appears to be the first time it has been used in this context. Our results are in favor of the presence of a phase transition from a localized state to an extended state for the electron as the phonon-electron coupling constant decreases. The phase transition manifests itself with a jump discontinuity in the potential energy as a function of the coupling constant and it affects the properties of the path of the electron in imaginary time: In the weak coupling regime the electron is in an extended state whereas in the strong coupling regime it is found in a self-trapped state.

==> def.tex <==
%%%%%%%%%% DEFINIZIONI %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pp}{{\mbox{\boldmath $p$}}}
\newcommand{\qq}{{\mbox{\boldmath $q$}}}
\newcommand{\kk}{{\mbox{\boldmath $k$}}}
\newcommand{\xx}{{\mbox{\boldmath $x$}}}
\newcommand{\xxb}{{\mbox{\boldmath $\overline{x}$}}}
\newcommand{\pint}{\int^{\!-}_{\!\!-}\!\!\!\!\!\int}
\newcommand{\bq}{\begin{eqnarray}}
\newcommand{\eq}{\end{eqnarray}}
\newcommand{\tpi}{\tilde{\pi}}
\newcommand{\cO}{{\cal O}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\nt}{\stackrel{\sim}{n}}
%\newcommand{\nt}{\mbox{$n$ \hspace{-1 em}\raisebox{1.1 ex}{$\sim$}}}
\newcommand{\pss}{\mbox{$\psi$ \hspace{-1 em}\raisebox{1.1 ex}{$\sim$}}}
\newcommand{\sgn}{{\rm sgn}}
\newcommand{\bji}{\mbox{${\rm J}_1$}}
\newcommand{\byi}{\mbox{${\rm Y}_1$}}
\newcommand{\bjii}{\mbox{${\rm J}_2$}}
\newcommand{\byii}{\mbox{${\rm Y}_2$}}
\newcommand{\bjo}{\mbox{${\rm J}_0$}}
\newcommand{\byo}{\mbox{${\rm Y}_0$}}
\newcommand{\fii}{\mbox{$F_I$}}
\newcommand{\chii}{\mbox{${{\chi_{}}_{}}_I$}}
\newcommand{\chio}{\mbox{${{\chi_{}}_{}}_o$}}
\newcommand{\up}{\stackrel}
\newcommand{\ams}{\AA}
\newcommand{\ro}{\overline{r}}
\newcommand{\rro}{\overline{{\bf r}}}
\newcommand{\rp}{r^\prime}
\newcommand{\sigmap}{\sigma^\prime}
\newcommand{\mpp}{m^\prime}
\newcommand{\mppp}{m^{\prime \prime}}
\newcommand{\mpppp}{m^{\prime \prime \prime}}
\newcommand{\rrp}{{\bf r}^\prime}
\newcommand{\kkp}{{\bf k}^\prime}
\newcommand{\vvp}{{\bf v}^\prime}
\newcommand{\qqp}{{\bf q}^\prime}
\newcommand{\rrpp}{{\bf r}^{\prime \prime}}
\newcommand{\Ro}{\overline{R}}
\newcommand{\Rp}{R^\prime}
\newcommand{\zp}{z^\prime}
\newcommand{\Vp}{V^\prime}
\newcommand{\KK}{{\bf K}}
\newcommand{\RR}{{\bf R}}
\newcommand{\ee}{{\bf e}}
\newcommand{\rr}{{\bf r}}
\newcommand{\kr}{{\cal K}}	
\newcommand{\ab}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\vv}{{\bf v}}
\newcommand{\uu}{{\bf u}}

\newcommand{\yy}{{\bf y}}

\newcommand{\xp}{x^\prime}
\newcommand{\zz}{{\bf z}}
\newcommand{\Rmi}{\mbox{$R_{m}^{i}$}}
\newcommand{\neo}[1]{\mbox{$n_o(\varepsilon_{#1})$}}
\newcommand{\eo}[1]{\mbox{$\varepsilon_{#1}$}}
\newcommand{\F}[4]{\mbox{${\bf F}_{\|}(R_{#1}^{#2}-R_{#3}^{#4})$}}
\newcommand{\FF}[4]{\mbox{${\bf F}(R_{#1}^{#2}-R_{#3}^{#4})$}}
\newcommand{\romo}{\mbox{$\rho_{m}({\bf r})$}}
\newcommand{\ron}{\mbox{$\rho(R^{1},\ldots,R^{n})$}}
\newcommand{\rot}{\mbox{$\rho_{T}$}}
\newcommand{\kp}{{\cal K}}
\newcommand{\roen}{\mbox{$\rho(R|R^{1},\ldots,R^{n})$}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\ba}{\begin{array}{ll}}
\newcommand{\ea}{\end{array}}
\newcommand{\et}{{\em et al}}
\newcommand{\re}{\rho_e}
\newcounter{ctr}
\newcounter{sbqi}
\def\lista{\begin{list}{(\roman{ctr})}{\usecounter{ctr}
\setlength{\rightmargin}{0.0truecm}\setlength{\leftmargin}{\labelwidth}}}
\def\appi{\renewcommand{\thesection}{Appendix \Alph{section}}}
\def\appf{\renewcommand{\thesection}{\Alph{section}}}
\def\subeqni{\addtocounter{equation}{1}\setcounter{sbqi}{\value{equation}}
\setcounter{equation}{0}\renewcommand{\theequation}
{\arabic{sbqi}\alph{equation}}}
\def\subeqnf{\setcounter{equation}{\value{sbqi}}
\renewcommand{\theequation}{\arabic{equation}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






